When waiting moves you in scoring combinatorial games

Combinatorial Scoring games, with the property `extra pass moves for a player does no harm', are characterized. The characterization involves an order embedding of Conway's Normal-play games. Also, we give a theorem for comparing games with scores (numbers) which extends Ettinger's work on dicot Scoring games.

==> cg-base.tex <==
\ProvidesFile{cg-base.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                          %%
%%              Raymond Chen's Game Builder                 %%
%%                  (somewhat altered)                      %%
%%                                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The \combgame macro takes as its argument the description of a game.
% It measures the size of the contents and scales all the slashes
% inside to the proper size.
%
% This makes eight passes over the input argument.
%
% For each of the four typestyles...
%
%   Typeset the argument in that style.
%   Set \cg@gamebox to an empty box with the height and depth of the game.
%       (During this first pass, \ifcg@drawbars is \iffalse.)
%   If we are in display style, set \cg@extension to the size of the
%       delimiter extension.  (If not, then set it to zero.)
%   Typeset the game proper, setting \ifcg@drawbars to \iftrue.
%
% This macro requires cooperation from the \cgslash, \cgsslash, etc. macros.

\newmuskip\cgslashmuskip
\cgslashmuskip=-2mu
\newlength\cgslashextension
\setlength\cgslashextension{1.5pt}

\def\cg@slashskip{\mskip\cgslashmuskip}

\newif\ifcg@star
\newif\ifcg@building\cg@buildingfalse
\newif\ifcg@drawbars\cg@drawbarsfalse
\newbox\cg@gamebox\setbox\cg@gamebox=\null
\newdimen\cg@extension
\newcounter{cg@readbarctr}

\newcommand\combgame{%
  \begingroup%
  \catcode`\|=\active%
  \cg@definebars%
  \@ifstar{\cg@startrue\cg@combgame}{\cg@starfalse\cg@combgame}%
}

\def\cg@combgame#1{%
  \mathpalette\cg@buildgame{#1}%
  \endgroup%
}

\def\cg@buildgame#1#2{%
    \begingroup%
    \cg@buildingtrue%
    \ifx#1\displaystyle%
      \ifcg@star%
        \cg@extension=0pt%
      \else%
        \cg@extension=\the\cgslashextension%
      \fi%
    \fi%
    \cg@drawbarsfalse%
    \setbox\z@\hbox{$#1#2$}%
    \ht\cg@gamebox\ht\z@%
    \dp\cg@gamebox\dp\z@%
    \cg@drawbarstrue%
    #1{#2}%
    \cg@buildingfalse%
    \endgroup%
}

\begingroup
\catcode`\|=\active
\gdef\cg@definebars{%
  \def|{\setcounter{cg@readbarctr}{1}\cg@readbars}%
  \def\{{\left\lbrace}
  \def\}{\right\rbrace}
}
\gdef\cg@readbars{%
  \@ifnextchar|{\stepcounter{cg@readbarctr}\cg@readnextbar}{\cgslashes{\thecg@readbarctr}}%
}
\gdef\cg@readnextbar|{\cg@readbars}
\endgroup

\newcommand\cgslash{\cgslashes{1}}
\newcommand\cgsslash{\cgslashes{2}}

\newcommand\cgslashes[2][]{%
  \ifcg@building
    \ifcg@drawbars
        \mathrel
        {\hbox{$%
    %% This part is deadly because \left and \right create implicit
    %% grouping.
        \toks\z@{}%
        \cg@loopmbars{#2}{\global\toks\z@\expandafter{\the\toks\z@\cg@mbarshelper}}%
        \def\cg@mbarshelper{\left\vert\mskip\cgslashmuskip}\the\toks\z@
            \mskip-\cgslashmuskip
            \@tempcnta#2\relax \advance\@tempcnta\m@ne
            \raise\@tempcnta\cg@extension\copy\cg@gamebox
            \lower\@tempcnta\cg@extension\copy\cg@gamebox
        \gdef\cg@mbarshelper{\right.}\the\toks\z@\n@space$}}%
    \else\mathrel\vert\fi
  \else
    \cg@badbar
  \fi
}

\def\cg@loopmbars#1#2{
    \@tempcnta#1\relax
    \loop
        #2%
        \advance\@tempcnta\m@ne
        \ifnum\@tempcnta>\z@
    \repeat
}

\def\cg@badbar{\errmessage{cgslash commands may only be used inside a combgame command.}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                          %%
%%                      Thermographs                        %%
%%                                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\define@key[cgk]{thermoplot}{left}{\def\cg@plot@left{#1}}
\define@key[cgk]{thermoplot}{right}{\def\cg@plot@right{#1}}
\define@key[cgk]{thermoplot}{top}{\def\cg@plot@top{#1}}
\define@key[cgk]{thermoplot}{bottom}{\def\cg@plot@bottom{#1}}
\define@key[cgk]{thermoplot}{scale}{\def\cg@plot@scale{#1}}
\define@key[cgk]{thermoplot}{axescolor}{\def\cg@plot@axescolor{#1}}
\define@key[cgk]{thermoplot}{clipmargin}{\def\cg@plot@clipmargin{#1}}
\define@key[cgk]{thermoplot}{baseline}{\def\cg@plot@baseline{#1}}
\define@key[cgk]{thermograph}{linecolor}{\def\cg@therm@linecolor{#1}}
\define@key[cgk]{thermograph}{displ}{\def\cg@therm@displ{#1}}

\newlength\cg@xorigin
\newlength\cg@yorigin
\newlength\cg@xsize
\newlength\cg@ysize
\newlength\cg@vcoord
\newlength\cg@tcoord

\newenvironment{thermoplot}[1][]{%
  \setkeys[cgk]{thermoplot}{left=2,right=-2,top=4,bottom=0,scale=1cm,axescolor=gray,clipmargin=6pt,baseline=0.0}%
  \setkeys[cgk]{thermoplot}{#1}%
  \setlength\cg@xorigin{\cg@plot@scale*\cg@plot@left}%
  \setlength\cg@yorigin{-\cg@plot@scale*\cg@plot@bottom}%
  \setlength\cg@xsize{\cg@plot@scale*\cg@plot@left-\cg@plot@scale*\cg@plot@right}%
  \setlength\cg@ysize{\cg@plot@scale*\cg@plot@top-\cg@plot@scale*\cg@plot@bottom}%
  \psset{xunit=-\cg@plot@scale,yunit=\cg@plot@scale}%
  \begin{pspicture}[\cg@plot@baseline](\the\cg@xsize,\the\cg@ysize)%
  {\color{\cg@plot@axescolor}%
   \psaxes[linecolor=\cg@plot@axescolor](\the\cg@xorigin,\the\cg@yorigin)(0,0)(\the\cg@xsize,\the\cg@ysize)}%
  \addtolength{\cg@xsize}{\cg@plot@clipmargin}\addtolength{\cg@ysize}{\cg@plot@clipmargin}%
  \psclip{\psframe[linecolor=white](-\cg@plot@clipmargin,-\cg@plot@clipmargin)(\the\cg@xsize,\the\cg@ysize)}%
}{%
  \endpsclip
  \end{pspicture}%
}%
\newcommand\trajectory[1][]{%
  \setkeys[cgk]{thermograph}{linecolor=black,displ=0pt}%
  \setkeys[cgk]{thermograph}{#1}%
  \def\cg@coords{{<-}}%
  \cg@readcoordsfortrajectory%
}
\newcommand\thermograph[2][]{%
  \setkeys[cgk]{thermograph}{linecolor=black,displ=0pt}%
  \setkeys[cgk]{thermograph}{#1}%
  \def\cg@therm@mast{#2}%
  \cg@starttrajectory%
  }
\def\cg@starttrajectory{%
  \cg@setvcoord{\cg@therm@mast}%
  \cg@settcoord{\cg@plot@top}%
  \addtolength{\cg@vcoord}{\cg@therm@displ}%
  \edef\cg@coords{{<-}(\the\cg@vcoord,\the\cg@tcoord)}%
  \cg@readcoordsfortrajectory%
}
\def\cg@readcoordsfortrajectory{%
  \@ifnextchar(\cg@readcoord%
    {\expandafter\cg@trajectoryline\cg@coords\cg@readnexttrajectory}%
}
\def\cg@trajectoryline{\psline[linecolor=\cg@therm@linecolor]}
\def\cg@readcoord(#1,#2){%
  \cg@setvcoord{#1}%
  \cg@settcoord{#2}%
  \addtolength{\cg@vcoord}{\cg@therm@displ}%
  \edef\cg@coords{\cg@coords(\the\cg@vcoord,\the\cg@tcoord)}%
  \cg@readcoordsfortrajectory%
}
\def\cg@settcoord#1{%
  \setlength\cg@tcoord{\cg@plot@scale*#1-\cg@plot@scale*\cg@plot@bottom}%
}
\def\cg@setvcoord#1{%
  \setlength\cg@vcoord{\cg@plot@scale*\cg@plot@left-\cg@plot@scale*#1}%
}
\def\cg@readnexttrajectory{\@ifnextchar;{\cg@eatsemicolon}{}}
\def\cg@eatsemicolon;{\cg@starttrajectory}



==> cg-board.tex <==
\ProvidesFile{cg-board.tex}
\newif\ifcg@board@trace%\cg@board@tracetrue % for debugging only

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Suggested for loony symbol:
% \usepackage{marvosym}\def\cgloony{\textrm\Moon}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FOR ALL DRAWING COMMANDS, USE pstricks COMMANDS.
%     \psunit IS SET, BUT \unitlength IS NOT SET.
% The general format for defining new board style is:
%   \newboard[options]{boardname}{code}
% There are numerous examples at the end of this file.
% For options, the following are allowed:
%
% code:  A sequence of character, expansion pairs (must have an even number of atoms)
%        default is X,x,L,l all make a black circle
%                   O,o,R,r all make a white circle
%                   .       is an empty square
%        The origin for an expansion is in the center of square; the expandsion is placed in a
%            makebox(0,0) so that any text is centered.
%        When defining a code for characters #, space, $, \, and ~,
%        quote them with a backslash.  (Do not prepend the \ in the
%        board diagram itself, though if you want to use space and \,
%        you'll need spaces=true.)
%
% unit:  Side length of a square (sets pstricks unit, access with \psunit)
% runit, xunit, yunit:  In case you want different x- and y-coordinate scales.
% linewidth:  Sets the pstricks linewidth
%
% text:  Sizing and style commands for text placed on a square.  (Example: StringsAndCoins)

% square:  What do use for a boardsquare.  (Use "square=" for no square.)
%          Default is a 1x1 square.
%          The origin for drawing the board square is in the lower
%          left corner of the square.  You can access counters
%          \cgboardrow and \cgboardcol to, for example, check parities (see Checkers).
% board:  What to draw for the gameboard.  Use counters cgboardrows and cgboardcols.
%         (Rarely needed;  Usually just draw each square individually as above.)
%         (see Hackenbush)
% frame: Put a frame around the board; generally used for debugging so you can see how large the
%         boards box is.
% printname:  (boolean) true means print the gamename under the board.  Default false.
%    (I use this for new games until such time as I've come up with distinctive pieces.)
%
% insert:  Stuff to insert in the diagram in addition to the gameboard.  Used to decorate the board.
% shrink: (boolean) Make the bounding box is .5 units smaller on each side.
% spaces: (boolean) Spaces and newlines are no longer whitespace (see Hex)
% color:  (boolean) Use color (currently implemented in Hackenbush, TopplingDominoes, Push, Shove)
%         Use \ifcgboardcolor to access
% 

% You can set these options in 4 different ways; suppose you are defining a new board named MyBoard.
% (1)  \newboard[...]{MyBoard}   --- When you defined your board
% (2)  \cgboardset{...}          --- This sets keys for all board types
% (3)  \MyBoardset{...}          --- A command is created by \newboard which appends ``set'' to your board name.
% (4)  \MyBoard[...]{xx\\oo\\}   --- When you make your board, you can define options in place.
% Note that the options are set in this order, and that \cgboardset obliterates the previous \cgboardset, and that
% \MyBoardset obliterates the previous \MyBoardset

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newboard
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \cg@board@extendcode\cg@board@basecode
\def\cgnewboard{\newboard}
\define@key[cgk]{board}{unit}{\psset{unit=#1}}
\define@key[cgk]{board}{xunit}{\psset{xunit=#1}}
\define@key[cgk]{board}{yunit}{\psset{yunit=#1}}
\define@key[cgk]{board}{runit}{\psset{runit=#1}}
\define@key[cgk]{board}{linewidth}{\psset{linewidth=#1}}
\define@key[cgk]{board}{text}[]{\def\cg@board@text{#1}}
\define@key[cgk]{board}{square}[\psline(0,0)(1,0)(1,1)(0,1)(0,0)]{\def\cg@board@square{#1}}
\define@key[cgk]{board}{frame}[\fbox]{\def\cg@board@frame{#1}}
\define@key[cgk]{board}{board}[]{\def\cg@board@theboard{#1}}
\define@key[cgk]{board}{printname}{\def\cg@board@printname{#1}}
\define@key[cgk]{board}{code}{\def\cg@board@extendcode{#1}}
\define@key[cgk]{board}{insert}{\def\cg@board@insertion{#1}}
\def\cgboardset#1{\def\cg@board@set{#1}}\def\cg@board@set{}

\define@boolkey[cgk]{board}{shrink}[true]{}
\define@boolkey[cgk]{board}{spaces}[true]{}
\define@boolkey[cgk]{board}{color}[true]{}

\newpsobject{cg@board@dottedline}{psline}{linestyle=dashed,dash=1.5pt 1.5pt}
\def\cg@board@default@keys{
   unit=.3cm,
   linewidth=.5pt,
   text=,
   square={\psline(0,0)(1,0)(1,1)(0,1)(0,0)},
   frame=,
   board=,
   printname=,
   code=,
   insert=,
   shrink=false,
   spaces=false,
   color=false
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Base gameboard code
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\cg@board@basecode{
x {\pscircle*{.45}}
o {\pscircle[fillstyle=solid,fillcolor=white]{.45}}
l {\cgboardalias{x}}
r {\cgboardalias{o}}
0 {0}
1 {1}
2 {2}
3 {3}
4 {4}
5 {5}
6 {6}
7 {7}
8 {8}
9 {9}
. {}
\ {\cgboardalias{.}}
\#{\cgnosquare}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% catcode stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\catcode`\#=11\gdef\cg@sharp{#}}
{\catcode`\$=11\gdef\cg@dollar{$}} % Second copy keeps file
{\catcode`\$=11\gdef\cg@dollar{$}} %  looking pretty in emacs
{\catcode`\~=11\gdef\cg@tilde{~}}
\begingroup
\catcode`|=0\catcode`\\=12|gdef|cg@backslash{\}
|endgroup
\def\cg@board@setcatcodes{%
  \catcode`\#=12%
  \catcode`\^=12%
  \catcode`\|=12%
  \catcode`\[=12%
  \catcode`\]=12%
  \catcode`\~=12\relax%
  \ifcgk@board@spaces
  \catcode`\\=12%
  \catcode`\ =12%
  \catcode`\^^M=12\relax%
  \fi%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Code stuff (i.e., the encoding of characters to board squares)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cgboardalias#1{%
  \@if@cg@board@code@defined{#1}%
  {\csname cg@board@code@#1\endcsname}%
  {\GenericWarning{}{Warning: Code for ``#1'' (an alias) unknown in game diagram}}}

\def\cg@board@set@code#1#2{
  \ifcg@board@trace\typeout{Setting ``\expandafter\string\csname cg@board@code@#1\endcsname'' to ``(not telling)''}\fi
  \expandafter\def\csname cg@board@code@#1\endcsname{#2}}
\def\cg@board@setstrings#1{\cg@board@buildsetstrings#1\cg@end\cg@end}
\def\cg@board@buildsetstrings#1#2{
  \ifx\cg@end#1
    \ifx\cg@end#2\let\next\relax
    \else\errmessage{combgames error: Mismatched arguments in board codes}
    \fi
  \else
    \ifx\\#1\cg@board@set@code{\cg@backslash}{#2}
    \else\ifx\ #1\cg@board@set@code{\space}{#2}
    \else\ifx#1\#\cg@board@set@code{\cg@sharp}{#2}
    \else\ifx\~#1\cg@board@set@code{\cg@tilde}{#2}
    \else\ifx\$#1\cg@board@set@code{\cg@dollar}{#2}
    \else\cg@board@set@code{#1}{#2}
    \fi\fi\fi\fi\fi
    \let\next\cg@board@buildsetstrings
  \fi
  \next
}

\def\cg@board@set@keys@#1{\expandafter\cg@board@set@keys\expandafter{#1}}
\def\cg@board@set@keys#1{\setkeys[cgk]{board}{#1}}
\newcommand\newboard[3][]{%
  \expandafter\newcommand\csname @cg@board@#2keys\endcsname{}%
  \expandafter\newcommand\csname #2set\endcsname[1]{%
    \expandafter\def\csname @cg@board@#2keys\endcsname{##1}}%
  \expandafter\newcommand\csname#2\endcsname[1][]{%
    %
    \ifmmode\def\cg@board@afterdone{}   % Force math mode if not in math mode
       \else\def\cg@board@afterdone{$}$ % (I forget why, mind you)
    \fi
    \begingroup%
    \expandafter\cg@board@set@keys\expandafter{\cg@board@default@keys}% Keys set in this file
    \setkeys[cgk]{board}{#1}% E.g., \newboard[...]{Domineering}
    \expandafter\cg@board@set@keys\expandafter{\cg@board@set}% \cgboardset{...}
    \expandafter\cg@board@set@keys@\expandafter{\csname @cg@board@#2keys\endcsname}% E.g., Domineeringset{...}
    \setkeys[cgk]{board}{##1}% E.g., \Domineering[...]{xo\\oo}
    \let\ifcgboardcolor=\ifcgk@board@color
    \expandafter\cg@board@buildsetstrings\cg@board@basecode\cg@end\cg@end
    \cg@board@setstrings{#3}%
    \expandafter\cg@board@buildsetstrings\cg@board@extendcode\cg@end\cg@end
    \begingroup%
    \cg@board@setcatcodes%
    \cg@board@read@the@board}}
\def\cg@board@read@the@board#1{\endgroup\cg@board@board{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Scanning and drawing the board
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{cgboardcol}
\newcounter{cgboardrow}
\newcounter{cgboardcols}
\newcounter{cgboardrows}

\def\cg@board@setdims#1{%
  \setcounter{cgboardcols}{0}\setcounter{cgboardcol}{0}\setcounter{cgboardrows}{0}%
                \cg@board@setdims@#1\end}%
\def\cg@board@advancerow{%%
  \ifnum\value{cgboardcols}<\value{cgboardcol} \setcounter{cgboardcols}{\value{cgboardcol}}\fi%
  \ifnum\value{cgboardcol}>0% Ignore leading newline (and the unlikely blank line)%
  \setcounter{cgboardcol}{0}%
  \refstepcounter{cgboardrows}\fi}%

{
\catcode`\^^M=12\relax%
\gdef\cg@board@setdims@#1{%
 \ifx#1\end%%
     \ifnum\value{cgboardcol}>0\cg@board@advancerow\fi% Append missing newline%
     \let\next=\relax%
 \else%
   % The following line must not end in a comment --- testing for newline
    \ifx#1
        \cg@board@advancerow%
    \else\ifx#1\\\cg@board@advancerow%
    \else\refstepcounter{cgboardcol}%
    \fi\fi%
 \let\next=\cg@board@setdims@\fi \next}}%

\def\cg@board@#1{%
  \psset{arrows=-}%
  \ifcgk@board@shrink\cg@board@decrementdims%
  \begin{pspicture}(.5,.5)(\arabic{cgboardcols}.5,\arabic{cgboardrows}.5)%
    \else%
    \begin{pspicture}(\arabic{cgboardcols},\arabic{cgboardrows})%
      \fi%
      \cg@board@theboard%
      \rput(0,-.1){\makebox(0,0)[lt]{\scriptsize\sc \cg@board@printname}}%
      \ifcgk@board@shrink\cg@board@incrementdims\fi%
      \cg@board@process{#1}%
      \cg@board@insertion%
    \end{pspicture}}%

\def\cg@board@incrementdims{%
  \addtocounter{cgboardrows}{1}%
  \addtocounter{cgboardcols}{1}}

\def\cg@board@decrementdims{%
  \addtocounter{cgboardrows}{-1}%
  \addtocounter{cgboardcols}{-1}}

\def\cg@board@process#1{%
  \setcounter{cgboardrow}{\value{cgboardrows}} \setcounter{cgboardcol}{0}  %
  \cg@board@process@#1\end%%
}
{
\catcode`\^^M=12\relax%
  \gdef\cg@board@process@#1{%
    \ifx#1\end%
  \let\next=\relax%
  \else%
   % first adjust row, col%
   % The following line must not end in a comment --- testing for newline
   \ifx#1
   \ifnum\value{cgboardcol}>0% Ignore leading newline (and the unlikely blank line)%
   \addtocounter{cgboardrow}{-1}\fi%
     \setcounter{cgboardcol}{0}%
   \else%
   \ifx#1\\%
   \ifnum\value{cgboardcol}>0% Ignore leading newline (and the unlikely blank line)%
   \addtocounter{cgboardrow}{-1}\fi%
     \setcounter{cgboardcol}{0}%
   \else%
     \addtocounter{cgboardcol}{1}%
   % what gets drawn is game specific
   \cg@board@displaychar{#1}%
   \fi\fi%
   % continue looping%
 \let\next=\cg@board@process@\fi \next}}%

\newlength{\cg@board@halfunit}

\def\cg@board@board#1{%
  \cg@board@setdims{#1}%
  \ifcgk@board@shrink\cg@board@decrementdims\fi%
  \setlength{\cg@board@halfunit}{.5\psyunit}%
  \setlength{\cg@board@halfunit}{\value{cgboardrows}\cg@board@halfunit}%
  \ifcgk@board@shrink\cg@board@incrementdims\fi%
  \raisebox{.5ex}{\raisebox{-1\cg@board@halfunit}%%
    {\expandafter\cg@board@frame%
      {\cg@board@%
        {#1}}}}\endgroup\cg@board@afterdone}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Processing characters of a cgboard
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@if@cg@board@code@defined#1#2#3{{\@ifundefined{cg@board@code@#1}{#3}{#2}}}

\def\cg@board@displaychar#1{%
  \@if@cg@board@code@defined{#1}%
  {\cg@board@display@char@#1}%
  {\lowercase{\@if@cg@board@code@defined{#1}}%
    {\lowercase{\cg@board@display@char@#1}}%
    {\GenericWarning{}{Warning: Code for ``#1'' unknown in game diagram}}}}

\newif\ifcg@board@drawsquare
\def\cgnosquare{\global\cg@board@drawsquarefalse}

\def\cg@board@display@char@#1{%
  \rput(\value{cgboardcol},\value{cgboardrow}){%
    \cg@board@drawsquaretrue%
    \rput(-.5,-.5){\makebox(0,0){\cg@board@text%
        {\ifcg@board@trace\typeout{Expanding ``\expandafter\string\csname cg@board@code@#1\endcsname''}\fi%
          \csname cg@board@code@#1\endcsname}}}%
    \rput(-1,-1){\ifcg@board@drawsquare\cg@board@square\fi}}}

\def\cg@board@drawsquare{{\rput(-.5,-.5){\cg@board@square}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THE GAMES DEFINED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DOMINEERING%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newboard[unit=.3cm,square=]{Domineering}{%%
  o {{\psline(-.5,-.5)(.5,-.5)(.5,.5)(-.5,.5)(-.5,-.5)}}%
  x {{\rput(0,0){{\pspolygon*[linewidth=0pt,linecolor=lightgray](-.5,-.5)(-.5,.5)(.5,.5)(.5,-.5)}}%
      \psline(-.5,-.5)(.5,-.5)(.5,.5)(-.5,.5)(-.5,-.5)}}%
  ^ {}%
  > {}%
  v {\psline(-.5,-.5)(.5,-.5)(.5,1.5)(-.5,1.5)(-.5,-.5)%%
      \rput(-.5,-.5){\pspolygon*[linewidth=0pt]%%
      (.4,.4)(.2,.2)(.8,.2)(.6,.4)(.6,1.6)(.8,1.8)(.2,1.8)(.4,1.6)}}%
  < {{\psline(-.5,-.5)(1.5,-.5)(1.5,.5)(-.5,.5)(-.5,-.5)}%
      \rput(-.5,-.5){\pspolygon*[linewidth=0pt]%
       (.4,.4)(.2,.2)(.2,.8)(.4,.6)(1.6,.6)(1.8,.8)(1.8,.2)(1.6,.4)}}%%
 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CLOBBER
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Clobber@Base#1#2{
  \SpecialCoor
  \rput(-.5,-.5){
    \psset{offset=0,nodesep=.1}
    \ifx#2a
    \pnode(.13333,.75){a}
    \pnode(.86666,-1|a){b}
    \pnode(.73333,.25){c}
    \pnode(.26666,-1|c){d}
    \pnode([angle=0]a){at}
    \pnode([angle=0]d){dt}
    \pnode([angle=-71.565,nodesep=.1]a){a1}
    \pnode([angle=180,nodesep=.05]c){c1}
    \pnode([angle=71.565]c){c2}
    \pnode([angle=108.435,nodesep=.1]dt){d2}
    \pnode([angle=-71.565,nodesep=.00]at){a2}
    \psarc(.5,.22){.08}{-240}{60}
    \else
    \pnode(.13333,.25){a}
    \pnode(.86666,-1|a){b}
    \pnode(.73333,.75){c}
    \pnode(.26666,-1|c){d}
    \pnode([angle=0]a){at}
    \pnode([angle=0]d){dt}
    \pnode([angle=71.565,nodesep=.1]a){a1}
    \pnode([angle=180,nodesep=.05]c){c1}
    \pnode([angle=-71.565]c){c2}
    \pnode([angle=-108.435,nodesep=.1]dt){d2}
    \pnode([angle=71.565,nodesep=.00]at){a2}
    \psarc(.5,.78){.08}{-60}{240}
    \fi
    \ifx#1O
    \pspolygon[linearc=.00](a1)(a2)(b)(c2)(c1)(d)
    \psset{linewidth=.015\psunit}
    \else
    \pspolygon[linearc=.00](a1)(a2)(b)(c2)(c1)(d)
    \pspolygon*[linearc=.00](a1)(a2)(b)(c2)(c1)(d)
    \psset{linecolor=white,linewidth=.5\pslinewidth}
    \fi
    \psline(d)(d2)(c2)(d2)(a2)
  }
}
\def\ClobberO{\Clobber@Base{O}{c}}
\def\ClobberX{\Clobber@Base{X}{c}}
\newboard[unit=.5cm]{Clobber}{
  x {\ClobberX}
  o {\ClobberO}
}
\newboard[unit=.3cm]{AntiClobber}{
  x {\Clobber@Base{X}{a}}
  o {\Clobber@Base{O}{a}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DOTS AND BOXES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newboard[square=,unit=.35cm,shrink=true,text=\bf]{DotsAndBoxes}{
  o {\pscircle*{.3}}
  - {\psline(-1,0)(1,0)\rput(-1,0){\cgboardalias{o}}}
  | {\psline(0,-1)(0,1)\rput(0,-1){\cgboardalias{o}}}
  : {\cg@board@dottedline(0,-1)(0,1)\rput(0,-1){\cgboardalias{o}}}
  + {\cg@board@dottedline(-1,0)(1,0)\rput(-1,0){\cgboardalias{o}}}
  * {\rput(-.05,0){\makebox(0,0){{$\cgloony$}}}}
  A {A}
  B {B}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% STRINGS AND COINS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\StringsAndCoinsCoin#1{\rput(0,0){#1}\rput(0,0){\pscircle{.5}}}
\newboard[square=,unit=.35cm,text=\bf\footnotesize]{StringsAndCoins}{
 o {\StringsAndCoinsCoin{\rm\$}}
 + {\cg@board@dottedline(-.45,0)(.45,0)}
 : {\cg@board@dottedline(0,-.45)(0,.45)}
 | {\psline(0,-.45)(0,.45)}
 * {\psline(-.45,0)(.45,0)\rput(-.05,.075){\makebox(0,0)[b]{$\cgloony$}}}
 - {\psline(-.45,0)(.45,0)}
 ! {\psline(0,-.45)(0,.45)\rput(-.05,0){\makebox(0,0)[l]{$\cgloony$}}}
 A {\StringsAndCoinsCoin{A}}
 B {\StringsAndCoinsCoin{B}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CHOMP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ChompPoison{\pscircle{.3}\psline(-.3,-.3)(.3,.3)\psline(-.3,.3)(.3,-.3)}
\newboard{Chomp}{
  o {}
  x {\cgboardalias{p}}
  p {\ChompPoison}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BRIDGIT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newboard[shrink=true,square=]{Bridgit}{
  o {\rput(0,0){\pscircle{.2}}}
  x {\rput(0,0){\pscircle*{.2}}}
  - {\psline(-.8,0)(.8,0)}
  | {\psline(0,-.8)(0,.8)}
  + {\cg@board@dottedline(-.8,0)(.8,0)}
  : {\cg@board@dottedline(0,-.8)(0,.8)}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AMAZONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\AmazonsArcher{%
  \psline[arrowsize=1\pslinewidth]{->}(.25,.25)(.8,.8)%
  \psline(.25,.8)(.3,.3)(.8,.25)%
  \psline[linewidth=1.5\pslinewidth](.2,.23)(.25,.25)(.23,.2)%
  \pscurve[linewidth=2\pslinewidth](.2,.8)(.675,.675)(.8,.2)}%
\def\AmazonsR{{\pscircle{.45}}\rput(-.5,-.5){\AmazonsArcher}}
\def\AmazonsL{{\pscircle*{.45}}{\psset{linecolor=white}\rput(-.5,-.5){\AmazonsArcher}}}
\newboard{Amazons}{
  o {}
  x {{\rput(0,0){{\pspolygon*[linewidth=0pt,linecolor=lightgray](-.5,-.5)(-.5,.5)(.5,.5)(.5,-.5)}}%
      \psline(-.5,-.5)(.5,-.5)(.5,.5)(-.5,.5)(-.5,-.5)}}%
  l {\AmazonsL}
  r {\AmazonsR}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SHOVE and PUSH
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\PushBase#1#2#3{
  \def\doit##1{%
    \ifcgboardcolor%
    \ifx#2O\pscurve*[linecolor=red]##1\pscurve##1%
    \else\ifx#2X\pscurve*[linecolor=blue]##1\pscurve##1%
    \else\pscurve*[linecolor=green]##1\pscurve##1%
    \fi\fi\else%
    \ifx#2O\pscurve##1%
    \else\ifx#2X\pscurve*##1%
    \else\pscurve*[linecolor=lightgray]##1\pscurve##1%
    \fi\fi\fi
  }
  \def\thepiece{
    \doit{(.55,.1)(.42,.2)(.33,.27)(.32,.3)(.33,.4)(.33,.5)(.33,.56)(.34,.6)(.355,.625)(.39,.625)
    (.39,.625)(.39,.625)(.39,.625)(.41,.8)(.425,.83)(.45,.83)(.465,.8)(.5,.4)(.525,.3)(.625,.22)}
    \ifx#2X
    \psecurve[linecolor=white,linewidth=.5\pslinewidth](.355,.625)(.39,.625)(.4,.6)(.4,.415)(.4,.425)
    \else
    \psecurve(.355,.625)(.39,.625)(.4,.6)(.4,.415)(.4,.425)
    \fi
    \psset{linewidth=.5\pslinewidth}
    \ifx#1P
    \psline(.6,.4)(.7,.4)
    \psline(.6,.7)(.7,.7)
    \else
    \psline(.7,.3)(.85,.3)
    \psline(.65,.45)(.9,.45)
    \psline(.65,.6)(.8,.6)
    \psline(.65,.75)(.9,.75)
    \fi}
  {
  \ifx#3a\psset{unit=.6\psunit}\fi
  \ifx#1P\rput(-.5,-.5){\thepiece}\else\rput(-.6,-.5){\thepiece}\fi
  }
}
\def\PushO{\PushBase{P}{O}{.}}
\def\PushX{\PushBase{P}{X}{.}}
\def\PushG{\PushBase{P}{G}{.}}
\def\ShoveO{\PushBase{S}{O}{.}}
\def\ShoveX{\PushBase{S}{X}{.}}
\def\ShoveG{\PushBase{S}{G}{.}}
\def\AllSmallPushO{\PushBase{P}{O}{a}}
\def\AllSmallPushX{\PushBase{P}{X}{a}}
\def\AllSmallPushG{\PushBase{P}{G}{a}}
\def\AllSmallShoveO{\PushBase{S}{O}{a}}
\def\AllSmallShoveX{\PushBase{S}{X}{a}}
\def\AllSmallShoveG{\PushBase{S}{G}{a}}
\newboard[unit=.5cm,square={\psline(0,0)(1,0)(1,1)(0,1)}]{Push}{
  . {}
  o {\PushO}
  O {\PushO}
  x {\PushX}
  X {\PushX}
  L {\PushX}
  R {\PushO}
  G {\PushG}
}
\newboard[unit=.5cm,square={\psline(0,0)(1,0)(1,1)(0,1)}]{Shove}{
  . {}
  o {\ShoveO}
  x {\ShoveX}
  g {\ShoveG}
}
\newboard[unit=.5cm,square={\psline(0,0)(1,0)(1,1)(0,1)}]{AllSmallShove}{
  . {}
  o {\AllSmallShoveO}
  x {\AllSmallShoveX}
  g {\AllSmallShoveG}
}
\newboard[unit=.5cm,square={\psline(0,0)(1,0)(1,1)(0,1)}]{AllSmallPush}{
  . {}
  o {\AllSmallPushO}
  x {\AllSmallPushX}
  g {\AllSmallPushG}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% HACKENBUSH STRINGS%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\hackred#1{%
  \ifcgboardcolor{\psset{linecolor=red,linewidth=4\pslinewidth}#1}%
  \else{\psset{doubleline=true,doublesep=1pt,linewidth=.5pt}#1}\fi}%
\def\hackblue#1{%
  \ifcgboardcolor{\psset{linecolor=blue,linewidth=4\pslinewidth}#1}%
  \else{\psset{linewidth=4\pslinewidth}#1}\fi}%
\def\hackgreen#1{%
  \ifcgboardcolor{\psset{linecolor=green,linewidth=4\pslinewidth}#1}%
  \else{\psset{linewidth=4\pslinewidth,linecolor=lightgray}#1}\fi}%

\def\hackedge{\psline(-.5,0)(.5,0)}
\def\Hackenbushstring@frame#1{\hspace{.15\psunit}#1\hspace{.15\psunit}}
\newboard[frame=\Hackenbushstring@frame,square={\rput(0,.5){\pscircle*{.15}}},unit=.5cm,xunit=.8cm,yunit=.3cm,%
         board={\psline[linewidth=8\pslinewidth,linecolor=lightgray](0,-.25)(0,\arabic{cgboardrows}.25)}]%
    {Hackenbushstring}{
  o {\hackred{\hackedge}\rput(.5,0){\pscircle*{.15}}\rput(-.5,0){\pscircle*{.15}}}
  x {\hackblue{\hackedge}\rput(.5,0){\pscircle*{.15}}\rput(-.5,0){\pscircle*{.15}}}
  b {\cgboardalias{x}}
  g {\hackgreen{\hackedge}\rput(.5,0){\pscircle*{.15}}\rput(-.5,0){\pscircle*{.15}}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TOPPLING DOMINOES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\DOMINO#1#2#3{\pspolygon#1[#3](-.2,-.5)(-.2,.3)(0,.5)(0,-.5)%
              \pspolygon#1[#3](0,-.5)(0,.5)(.2,.5)(.2,-.5)%
              \psline[#2](0,0)(-.2,-.1)}
\newboard[xunit=.3cm,yunit=.6cm,square=,%
         board={\psline[linewidth=6\pslinewidth,linecolor=lightgray](0,0)(\arabic{cgboardcols},0)}]
        {TopplingDominoes}{
          x {\ifcgboardcolor\DOMINO{}{}{fillcolor=blue,fillstyle=solid}\else\DOMINO{*}{linecolor=white}{}\fi}
          o {\ifcgboardcolor\DOMINO{}{}{fillcolor=red,fillstyle=solid}\else\DOMINO{}{}{}\fi}
          g {\ifcgboardcolor\DOMINO{}{}{fillcolor=green,fillstyle=solid}\else\DOMINO{}{}{fillcolor=lightgray,fillstyle=solid}\fi}
        }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% HEX
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\HexHexagon{\rput(0,0){\psline(-.666666,0)(-.333333,1)(.333333,1)(.666666,0)(.3333333,-1)(-.3333333,-1)(-.666666,0)}}
\def\HexBlack{\rput(0,0){\pscircle*{.5}}}
\def\HexWhite{\rput(0,0){\pscircle{.5}}\rput(0,0){\pscircle{.2}}}
\newlength{\Hexunit}
\setlength{\Hexunit}{.125cm}
\newboard[square=,runit=1.3\Hexunit,xunit=1.73206\Hexunit,yunit=1\Hexunit,spaces]{Hex}{
  o {\HexHexagon}
  * {\HexHexagon}
  l {\HexBlack}
  r {\HexWhite}
  x {\HexHexagon\HexBlack}
  o {\HexHexagon\HexWhite}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MAZE and MAIZE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newboard[square=,unit=.2cm,shrink,spaces]{Maze}{
  L {$\L$} R {$\R$} N {$\N$} P {$\P$}
  o {}
  * {\psline(-.05,-.05)(.05,.05)\psline(-.05,.05)(.05,-.05)}
  x {\pscircle{.8}\rput(0,0){\rput(0,0){$\star$}}}
  / {\psline(-1,-1)(1,1)}
 \\ {\psline(-1,1)(1,-1)}
}
\newboard[square=,unit=.2cm,shrink,spaces]{Maize}{
  L {$\L$} R {$\R$} N {$\N$} P {$\P$}
  o {}
  * {\psline(-.05,-.05)(.05,.05)\psline(-.05,.05)(.05,-.05)}
  x {\pscircle{.8}\pscircle*{.1}}
  / {\psline(-1,-1)(1,1)}
 \\ {\psline(-1,1)(1,-1)}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CHECKERS
% Checkers is not yet complete --- needs a King --- provided here only
%  to provide an example of using counters cgboardrow and cgboardcol
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\CheckersSquare{ 
  \@tempcnta=\value{cgboardrow}
  \advance\@tempcnta\value{cgboardcol}
  \ifodd\@tempcnta
  {\pspolygon(0,0)(1,0)(1,1)(0,1)}\else
  {\pspolygon[fillcolor=lightgray,fillstyle=solid](0,0)(1,0)(1,1)(0,1)}\fi
}

\newboard[square=.]{Checkers}{ % Since a square is drawn after the
  % piece, Checkers requires us to draw the square explicitly.
  . {\rput(-.5,-.5){\CheckersSquare}}
  x {\cgboardalias{.}\pscircle*{.4}}
  o {\cgboardalias{.}\pscircle[fillstyle=solid,fillcolor=white]{.4}}
}


==> graphs_config.tex <==
% Local configuration for version 1.53 of graphs.sty. Frank Drewes, 16.11 2003

% The \special macro below must contain the path under which the file
% graphs.header can be found in you local installation. Please modify it
% accordingly.

\special{header=graphs.header}


==> graphs_ps.tex <==
% `special' commands for version 1.53 of graphs.sty. Frank Drewes, 16/11 2003

\def\ps@s{ }
\def\ps@convertnum#1{
	#1 \number\unitlength\ps@s mul 65536 div 72.27 div 72 mul
}

%-----------------------------------------------------------------------------%


\def\ps@rectangle[#1,#2]{% width, height
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		[ \g@ncolour\ps@s\g@ncolourmod ]\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\iffillednodes true \else false\fi\ps@s
		psrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@circle[#1]{% diameter
\special{"	\ps@convertnum{#1}
		[ \g@ncolour\ps@s\g@ncolourmod ]\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\iffillednodes true \else false\fi\ps@s
		pscircle}}

%-----------------------------------------------------------------------------%

\def\ps@line(#1,#2){% end x, end y
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\g@ldash\ps@s
		psline}}

%-----------------------------------------------------------------------------%

\def\ps@loopA(#1,#2)(#3,#4){% from (#1,#2) to (#3,#4)
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psloop}}

%-----------------------------------------------------------------------------%

\def\ps@loopB#1(#2,#3){% angle #1, axis (#2,#3)
\special{"	#1
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		psloopbyangle
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psloop}}
		
%-----------------------------------------------------------------------------%

\def\ps@looparrowonrectangleA(#1,#2)(#3,#4)[#5,#6]{% 
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		\ps@convertnum{#5}
		\ps@convertnum{#6}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowonrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@looparrowoncircleA(#1,#2)(#3,#4)[#5]{% 
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		\ps@convertnum{#5}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@looparrowonrectangleB#1(#2,#3)[#4,#5]{% 
\special{"	#1
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		psloopbyangle
		\ps@convertnum{#4}
		\ps@convertnum{#5}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowonrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@looparrowoncircleB#1(#2,#3)[#4]{% 
\special{"	#1
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		psloopbyangle
		\ps@convertnum{#4}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@deletebox(#1,#2){% width, height in scaled points
\special{"	#1 65536 div
		#2 65536 div
		psdeletebox}}

%-----------------------------------------------------------------------------%

\def\ps@arrowonrectangle(#1,#2) [#3,#4]{% x, y, width, height
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psarrowonrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@arrowoncircle(#1,#2) [#3]{% x, y, diameter of circle
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psarrowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@path(#1,#2)#3{% start coordinates, (xi,yi[,di]) ...
	\def\extractvalues(##1)##2;{%
	  \ifx\endmarker##1\else%
	    \extractvalues##2;\extractvals(##1,0,)%
	  \fi}%
	\def\extractvals(##1,##2,##3,##4){%
	  \ps@convertnum{##1}%
	  \ps@convertnum{##2}%
	  ##3%
	}%
	\special{" mark \extractvalues#3(\endmarker);
			\ps@convertnum{#1}
			\ps@convertnum{#2}
			\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
			[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
			\g@ldash\ps@s
			[ \g@fcolour\ps@s\g@fcolourmod ]\ps@s
			\iffilledareas true \else false\fi\ps@s pspath}}

%-----------------------------------------------------------------------------%

\def\ps@curve#1#2{% base length, (x1,y1,ang1[factor1]) ...
	\def\extractvalues(##1(##2;##3{%
	  \ifx\endmarker##1\else%
	    \extractvalues(##2;{##3}\extractvals(##1[##3,##3];%
	  \fi}%
	\def\extractvals(##1,##2,##3)[##4,##5]##6;{%
	  ##5\ps@s
	  ##4\ps@s
	  ##3\ps@s
	  \ps@convertnum{##2}%
	  \ps@convertnum{##1}%
	}%
	\special{" mark \extractvalues#2(\endmarker(;{#1}
			\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
			[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
			\g@ldash\ps@s
			[ \g@fcolour\ps@s\g@fcolourmod ]\ps@s
			\iffilledareas true \else false\fi\ps@s pscurve}}

%-----------------------------------------------------------------------------%

\def\ps@bubble#1#2{% length factor, (x1,y1) ...
	\def\extractvalues(##1)##2;{%
	  \ifx\endmarker##1\else%
	    \extractvalues##2;\extractvals(##1)%
	  \fi}%
	\def\extractvals(##1,##2){%
	  \ps@convertnum{##2}%
	  \ps@convertnum{##1}%
	}%
	\special{" mark \extractvalues#2(\endmarker);
			#1\ps@s
			\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
			[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
			\g@ldash\ps@s
			[ \g@fcolour\ps@s\g@fcolourmod ]\ps@s
			\iffilledareas true \else false\fi\ps@s psbubble}}

%-----------------------------------------------------------------------------%

\def\ps@dirbowoncircle(#1,#2)(#3,#4,#5)[#6]{% (x1,x2) (y1,y2,d), radius
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		#5\ps@s
		\ps@convertnum{#6}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\g@ldash\ps@s
		psdirbowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@dirbowonrectangle(#1,#2)(#3,#4,#5)[#6,#7]{% (x1,x2) (y1,y2,d),
                                                  % xsize, ysize
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		#5\ps@s
		\ps@convertnum{#6}
		\ps@convertnum{#7}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\g@ldash\ps@s
		psdirbowonrectangle}}

%-----------------------------------------------------------------------------%


